Formal Verification for Blockchain-based Insurance Claims Processing

Insurance claims processing involves multi-domain entities and multi-source data, along with a number of human-agent interactions. Use of Blockchain technology-based platform can significantly improve scalability and response time for processing of claims which are otherwise manually-intensive and time-consuming. However, the chaincodes involved within the processes that issue claims, approve or deny them as required, need to be formally verified to ensure secure and reliable processing of transactions in Blockchain. In this paper, we use a formal modeling approach to verify various processes and their underlying chaincodes relating to different stages in insurance claims processing viz., issuance, approval, denial, and flagging for fraud investigation by using linear temporal logic (LTL). We simulate the formalism on the chaincodes and analyze the breach of chaincodes via model checking.

==> AttackTree/Attacktree.tex <==
\centering
% \small
    \begin{adjustbox}{width=0.85\textwidth}
\begin{tikzpicture}[
 % Gates and symbols style
    and/.style={and gate US,thick,draw,fill=red!60,rotate=90,
		anchor=east,xshift=-1mm},
    or/.style={or gate US,thick,draw,fill=blue!60,rotate=90,anchor=east,xshift=-1mm},
% Label style
    label distance=3mm,
    every label/.style={blue},
% Event style
    event/.style={rectangle,thick,draw,fill=yellow!20,text width=2.5cm,
		text centered,font=\sffamily,anchor=north},
% Children and edges style
    edge from parent/.style={very thick,draw=black!70},
    edge from parent path={(\tikzparentnode.south) -- ++(0,-1.05cm)
			-| (\tikzchildnode.north)},
    level 1/.style={sibling distance=6cm,level distance=1.5cm,
			growth parent anchor=south,nodes=event},
    level 2/.style={sibling distance=5cm, level distance=1.5cm},
    level 3/.style={sibling distance=3cm, level distance=1.5cm},
    level 4/.style={sibling distance=2cm, level distance=1.5cm}
    level 5/.style={sibling distance=2cm, level distance=1.5cm}
%%  For compatability with PGF CVS add the absolute option:
%   absolute
    ]
%% Draw events and edges
\node (g1) [event] {LoI for ClaimChain}
    child[level distance=1.3cm, sibling distance=8.5cm]
    {node (g2) {System Compromise}
    child[sibling distance=5.5cm, level distance=1cm]{node (t1) {Sybil attack to crowd \\ out honest users}
    child[level distance=1.4cm, sibling distance=30mm]{node (s1) {Obtain legitimate \\ user accounts}
    }
    child[level distance=1.4cm, sibling distance=30mm]{node (s2) {Create malicious \\ user accounts}}
    }
    % child[sibling distance=40mm, level distance=1.3cm]{node (t2){Fraudulent Claims}
    % child[sibling distance=30mm, level distance=1.3cm]{node (s3) {Duplicate Claims}}
    % child[sibling distance=30mm, level distance=1.3cm]{node (s4) {Claim Misinformation}}
    % }
    % child[level distance=1.3cm, sibling distance=40mm]{node (t3) {Sybil attack to crowd out honest nodes}
    % }
    %  child[sibling distance=40mm, level distance=1.3cm]{node (t3){Timestamp Manipulation}
    % child[sibling distance=30mm, level distance=1.3cm]{node (s3) {Attacker login}}
    % child[sibling distance=30mm, level distance=1.3cm]{node (s4) {Access to the Blockchain Transaction}}
    % }
    }
    child[level distance=1.3cm, sibling distance=8.5cm]
    {node (g2) {Data Modification}
    % child[sibling distance=5.5cm, level distance=1.4cm]{node (t1) {Injection Attack}
    % child[level distance=1.3cm, sibling distance=30mm]{node (s1) {Getting access to the Blockchain}
    % }
    % child[sibling distance=26mm, level distance=1.9cm]{node (s2) {Sending malicious data as transaction}}
    % }
    child[sibling distance=50mm, level distance=1.3cm]{node (t2){SQL Injection}
    child[sibling distance=30mm, level distance=1.3cm]{node (s3) {Leverage exposed \\ input tags}}
    child[sibling distance=30mm, level distance=1.3cm]{node (s4) {SQL modification \\ commands}}
    }
    % child[level distance=1.3cm, sibling distance=40mm]{node (t3) {Sybil attack to crowd out honest nodes}
    % }
     child[sibling distance=50mm, level distance=1.3cm]{node (t3){Timestamp Manipulation}
    child[sibling distance=30mm, level distance=3cm]{node (s3) {Attacker login}}
    child[sibling distance=30mm, level distance=2cm]{node (s4) {Access to the Blockchain Transaction}}
    }
    }
    child[level distance=1.3cm, sibling distance=10cm]{node(g3){Application Compromise}
    child[sibling distance=40mm, level distance=1.3cm]{node (t4) {Install Malware to server}
    child[level distance=2.2cm, sibling distance=18mm]{node {Unauthorized access}
    child[level distance=1cm, sibling distance=48mm]{node (l1) {Phishing for user credentials}
    child[level distance=1.3cm, sibling distance=48mm]{node (s1) {Launch Email}}
    child[sibling distance=48mm, level distance=1.3cm]{node (s2) {Shoots text
 message}}
    }
    % child[sibling distance=10mm, level distance=1.3cm]{node (l2) {Analyze packets}}
    }
    child[level distance=2.2cm, sibling distance=40mm]{node (s6) {Insertion of malicious software}
    }
    }
    child[level distance=1.3cm, sibling distance=80mm]{node (s6) {Fraudulent \\ Claims}
    child[level distance=1.3cm, sibling distance=30mm]{node {Duplicate \\ Claims }}
    child[sibling distance=30mm, level distance=1.3cm]{node (l2) {Claim \\ Misinformation }}
    }
    };
%% Place gates and other symbols
%% In the CVS version of PGF labels are placed differently than in PGF 2.0
%% To render them correctly replace '-20' with 'right' and add the 'absolute'
%% option to the tikzpicture environment. The absolute option makes the 
%% node labels ignore the rotation of the parent node.
    \node [or] at (g1.south) [] {};
    \node [or] at (g2.south) [] {};
    \node [or] at (g3.south) [] {};
        %\draw[>=latex,->] (g3.north) to (g3.south);
    %\node [or] at (g3.south) [] {};
    \node [or] at (t1.south) [] {};
        % \draw[>=latex,->] (t1.north) to (t1.south);
    \node [and] at (t3.south) [] {};
    %\node [or] at (t2.south) [] {};
    \node [and] at (t2.south) (t2) [] {};
    %   \draw[>=latex,->] (t2.north) to (t2.south);
    % \node [and] at (s5.south) [] {};
        % \draw[>=latex,->] (s5.north) to (s5.south);
       \node [and] at (t4.south) (t4) [] {};
        \draw[>=latex,->] (t4.north) to (t4.south);  
        \node [or] at (l1.south) [] {};
    \node [or] at (s6.south) [] {};
        % \draw[>=latex,->] (s6.north) to (s6.south);
    %\node [or] at (s4.south) [] {};
    %\node [or] at (s7.south) [] {};
\end{tikzpicture}
\end{adjustbox}
\caption{{Security Attack tree for Loss of Integrity issues in ClaimChain.}}
\label{fig:AT1}
\vspace{1mm}
\normalsize

==> AttackTree/LoA.tex <==
\centering
\begin{adjustbox}{width=0.8\textwidth}
\begin{tikzpicture}[
 % Gates and symbols style
    and/.style={and gate US,thick,draw,fill=red!60,rotate=90,
		anchor=east,xshift=-1mm},
    or/.style={or gate US,thick,draw,fill=blue!60,rotate=90,anchor=east,xshift=-1mm},
% Label style
    label distance=3mm,
    every label/.style={blue},
% Event style
    event/.style={rectangle,thick,draw,fill=yellow!20,text width=2cm,
		text centered,font=\sffamily,anchor=north},
% Children and edges style
    edge from parent/.style={very thick,draw=black!70},
    edge from parent path={(\tikzparentnode.south) -- ++(0,-1.05cm)
			-| (\tikzchildnode.north)},
    level 1/.style={sibling distance=6cm,level distance=1.5cm,
			growth parent anchor=south,nodes=event},
    level 2/.style={sibling distance=5cm, level distance=1.5cm},
    level 3/.style={sibling distance=3cm, level distance=1.5cm},
    level 4/.style={sibling distance=2cm, level distance=1.5cm}
    level 5/.style={sibling distance=2cm, level distance=1.5cm}
%%  For compatability with PGF CVS add the absolute option:
%   absolute
    ]
%% Draw events and edges
\node (g1) [event] {LoA for\\ClaimChain}
    child[sibling distance=10cm]{node (g2) {DOS Compromise \\ System Availability}
    child[sibling distance=5.5cm]{node (t1) {Packet \\ Spoofing}
    child[sibling distance=30mm]{node (l1) {Organize \\ botnet}}
     child[sibling distance=40mm, level distance=1.5cm]{node (l2) {Identify an \\ exposed service}}
    }
    child[sibling distance=60mm, level distance=2cm]{node (t2){Syn Flood \\Scenario}
    child{node (s3) {Sending SYN packets}}
    child[level distance=2.3cm]{node (s4) {Targeting devices}}
    }
    }
    child[sibling distance=10cm]{node(g3){APT compromises \\ system resources}
    child[sibling distance=20mm, level distance=1.5cm]{node (t3) {Cryptojacking
    %Eavesdropping
    }
    child[level distance=2cm, sibling distance=16mm]{node (s5) {Access System \\ resources}
     child[sibling distance=30mm]{node (l1) {Phishing}}
     child[sibling distance=40mm, level distance=1.5cm]{node (l2) {Get system \\ credentials}}
    }
    child[sibling distance=40mm]{node (s6) {Malicious Code \\ Injection}
    % child[sibling distance=18mm]{node (l3) {Intrusion}}
    % child[sibling distance=50mm]{node (l4) {Eavesdropping}}
    }
    }
    child[sibling distance=75mm]{node (t4) {Ransomware}
     child[sibling distance=5mm]{node (l3) {Access System \\ resources}
     child[sibling distance=18mm]{node {Phishing}}
    child[sibling distance=50mm]{node (l4) {Get system \\ credentials}}}
    child[sibling distance=50mm]{node (l4) {Data encryption}}
    }};
%% Place gates and other symbols
%% In the CVS version of PGF labels are placed differently than in PGF 2.0
%% To render them correctly replace '-20' with 'right' and add the 'absolute'
%% option to the tikzpicture environment. The absolute option makes the 
%% node labels ignore the rotation of the parent node.
    \node [or] at (g1.south) [] {};
    \node [or] at (g2.south) [] {};
    \node [or] at (g3.south)(g3) [] {};
        % \draw[>=latex,->] (g3.north) to (g3.south);
    %\node [or] at (g3.south) [] {};
    \node [and] at (t1.south)(t1) [] {};
        % \draw[>=latex,->] (t1.north) to (t1.south);
    \node [or] at (t3.south) [] {};
    \node [and] at (l3.south) [] {};
    \node [and] at (t4.south) [] {};
    \node [and] at (t2.south) (t2) [] {};
    %   \draw[>=latex,->] (t2.north) to (t2.south);
    \node [and] at (s5.south) (s5) [] {};
        % \draw[>=latex,->] (s5.north) to (s5.south);
    % \node [and] at (s6.south) (s6) [] {};
        % \draw[>=latex,->] (s6.north) to (s6.south);
    %\node [or] at (s4.south) [] {};
    %\node [or] at (s7.south) [] {};
\end{tikzpicture}
\end{adjustbox}
\caption{Attack tree for Loss of Availability in ClaimChain architecture}
\vspace{5mm}
\label{fig:AT2}


==> AttackTree/PrivacyAttackTree.tex <==
\centering
\begin{adjustbox}{width=0.8\textwidth}
\begin{tikzpicture}[
 % Gates and symbols style
    and/.style={and gate US,thick,draw,fill=red!60,rotate=90,
		anchor=east,xshift=-1mm},
    or/.style={or gate US,thick,draw,fill=blue!60,rotate=90,anchor=east,xshift=-1mm},
% Label style
    label distance=3mm,
    every label/.style={blue},
% Event style
    event/.style={rectangle,thick,draw,fill=yellow!20,text width=2cm,
		text centered,font=\sffamily,anchor=north},
% Children and edges style
    edge from parent/.style={very thick,draw=black!70},
    edge from parent path={(\tikzparentnode.south) -- ++(0,-1.05cm)
			-| (\tikzchildnode.north)},
    level 1/.style={sibling distance=6cm,level distance=1.5cm,
			growth parent anchor=south,nodes=event},
    level 2/.style={sibling distance=5cm, level distance=1.5cm},
    level 3/.style={sibling distance=3cm, level distance=1.5cm},
    level 4/.style={sibling distance=2cm, level distance=1.5cm}
    level 5/.style={sibling distance=2cm, level distance=1.5cm}
%%  For compatability with PGF CVS add the absolute option:
%   absolute
    ]
%% Draw events and edges
\node (g1) [event] {LoC for \\ClaimChain}
    child[sibling distance=8.5cm]{node (g2) {Unauthorized Access\\ to User's Info}
    child[sibling distance=5.5cm]{node (t1) {Man in \\ the middle}
    child[sibling distance=30mm]{node (s1) {Capture\\Packets}
    }
    child[sibling distance=20mm, level distance=1.5cm]{node (s2) {Analyze\\ Packets}}
    }
    child[sibling distance=40mm, level distance=1.5cm]{node (t2){Attack \\Scenario}
    child{node (s3) {Eavesdropping}}
    child[level distance=1.5cm]{node (s4) {Intrusion}
    child[sibling distance=30mm, level distance=1.5cm]{node (l1) {Phishing}}
     child[sibling distance=40mm, level distance=1.5cm]{node (l2) {Get System \\ Credentials }}}
    }
    }
    child[sibling distance=8.5cm]{node(g3){Unauthorized Access\\ to Database}
    child[sibling distance=12.5mm, level distance=1.5cm]{node (t3) {SQL\\ Injection
    %Eavesdropping
    }
    child[level distance=1.5cm, sibling distance=16mm]{node (s5) {Leverage Exposed \\ Input Tags}
    %   child[sibling distance=30mm]{node (l1) {Capture\\packets}}
    %   child[sibling distance=40mm, level distance=1.5cm]{node (l2) {Analyze\\packets}}
    }
    child[sibling distance=40mm]{node (s6) {SQL Select\\Commands}
    %  child[sibling distance=18mm]{node (l3) {Intrusion}
    % }
    % child[sibling distance=50mm]{node (l4) {Eavesdropping}}
    }
    }
    child[sibling distance=90mm]{node (t4) {External connection \\ to Database}
    child[sibling distance=18mm]{node {Phishing for \\ misaligned ports}
    }
    child[sibling distance=40mm]{node (l4) {Leverage system \\ failure}
    child[sibling distance=25mm]{node {Identify connected \\ service and port}
    }
    child[sibling distance=25mm]{node {Vacate \\ the port}
    }
    }}
    };
%% Place gates and other symbols
%% In the CVS version of PGF labels are placed differently than in PGF 2.0
%% To render them correctly replace '-20' with 'right' and add the 'absolute'
%% option to the tikzpicture environment. The absolute option makes the 
%% node labels ignore the rotation of the parent node.
    \node [or] at (g1.south) [] {};
    \node [or] at (g2.south) [] {};
    \node [or] at (g3.south)(g3) [] {};
        % \draw[>=latex,->] (g3.north) to (g3.south);
    %\node [or] at (g3.south) [] {};
    \node [and] at (t1.south)(t1) [] {};
        % \draw[>=latex,->] (t1.north) to (t1.south);
    \node [and] at (t3.south) [] {};
    \node [or] at (t4.south) [] {};
    \node [and] at (t2.south) (t2) [] {};
    %   \draw[>=latex,->] (t2.north) to (t2.south);
    \node [and] at (s4.south) [] {};
     \node [and] at (l4.south) [] {};
        % \draw[>=latex,->] (s5.north) to (s5.south);
    % \node [and] at (s6.south) (s6) [] {};
        % \draw[>=latex,->] (s6.north) to (s6.south);
    %\node [or] at (s4.south) [] {};
    %\node [or] at (s7.south) [] {};
\end{tikzpicture}
\end{adjustbox}
 \caption{Attack tree for Loss of Confidentiality in ClaimChain architecture}
\vspace{2mm}
\label{fig:AT3}


==> AttackTree/attackmodel.tex <==
\centering
    \begin{adjustbox}{width=0.9\textwidth}
\begin{tikzpicture}[
 % Gates and symbols style
    and/.style={and gate US,thick,draw,fill=red!60,rotate=90,
		anchor=east,xshift=-1mm},
    or/.style={or gate US,thick,draw,fill=blue!60,rotate=90,anchor=east,xshift=-1mm},
% Label style
    label distance=3mm,
    every label/.style={blue},
% Event style
    event/.style={rectangle,thick,draw,fill=yellow!20,text width=2.5cm,
		text centered,font=\sffamily,anchor=north},
% Children and edges style
    edge from parent/.style={very thick,draw=black!70},
    edge from parent path={(\tikzparentnode.south) -- ++(0,-1.05cm)
			-| (\tikzchildnode.north)},
    level 1/.style={sibling distance=6cm,level distance=1.5cm,
			growth parent anchor=south,nodes=event},
    level 2/.style={sibling distance=5cm, level distance=1.5cm},
    level 3/.style={sibling distance=3cm, level distance=1.5cm},
    level 4/.style={sibling distance=2cm, level distance=1.5cm}
    level 5/.style={sibling distance=2cm, level distance=1.5cm}
%%  For compatability with PGF CVS add the absolute option:
%   absolute
    ]
%% Draw events and edges
\node (g1) [event] {G}
    child[level distance=1.3cm, sibling distance=8.5cm]
    {node (g2) {$M_1$}
    child[sibling distance=5.5cm, level distance=1.4cm]{node (t1) {$M_4$}
    child[level distance=1.3cm, sibling distance=30mm]{node (s1) {$x_1$}
    }
    child[sibling distance=26mm, level distance=1.9cm]{node (s2) {$x_2$}}
    }
    % child[sibling distance=40mm, level distance=1.3cm]{node (t2){Fraudulent Claims}
    % child[sibling distance=30mm, level distance=1.3cm]{node (s3) {Duplicate Claims}}
    % child[sibling distance=30mm, level distance=1.3cm]{node (s4) {Claim Misinformation}}
    % }
    % child[level distance=1.3cm, sibling distance=40mm]{node (t3) {Sybil attack to crowd out honest nodes}
    % }
    %  child[sibling distance=40mm, level distance=1.3cm]{node (t3){Timestamp Manipulation}
    % child[sibling distance=30mm, level distance=1.3cm]{node (s3) {Attacker login}}
    % child[sibling distance=30mm, level distance=1.3cm]{node (s4) {Access to the Blockchain Transaction}}
    % }
    }
    child[level distance=1.3cm, sibling distance=8.5cm]
    {node (g2) {$M_2$}
    % child[sibling distance=5.5cm, level distance=1.4cm]{node (t1) {Injection Attack}
    % child[level distance=1.3cm, sibling distance=30mm]{node (s1) {Getting access to the Blockchain}
    % }
    % child[sibling distance=26mm, level distance=1.9cm]{node (s2) {Sending malicious data as transaction}}
    % }
    child[sibling distance=50mm, level distance=1.3cm]{node (t2){$M_5$}
    child[sibling distance=30mm, level distance=1.3cm]{node (s3) {$x_3$}}
    child[sibling distance=30mm, level distance=1.3cm]{node (s4) {$x_4$}}
    }
    % child[level distance=1.3cm, sibling distance=40mm]{node (t3) {Sybil attack to crowd out honest nodes}
    % }
     child[sibling distance=50mm, level distance=1.3cm]{node (t3){$M_6$}
    child[sibling distance=30mm, level distance=1.7cm]{node (s3) {$x_5$}}
    child[sibling distance=30mm, level distance=1.3cm]{node (s4) {$x_6$}}
    }
    }
    child[level distance=1.3cm, sibling distance=10cm]{node(g3){$M_3$}
    child[sibling distance=40mm, level distance=1.3cm]{node (t4) {$M_7$}
    child[level distance=1.2cm, sibling distance=16mm]{node {$M_9$}
    child[level distance=1.3cm, sibling distance=48mm]{node (l1) {$M_{10}$}
    child[level distance=1.3cm, sibling distance=48mm]{node (s1) {$x_{10}$}}
    child[sibling distance=10mm, level distance=1.3cm]{node (s2) {$x_{11}$}}
    }
    % child[sibling distance=10mm, level distance=1.3cm]{node (l2) {Analyze packets}}
    }
    child[level distance=1.3cm, sibling distance=40mm]{node (s6) {$x_7$}
    }
    }
    child[level distance=1.3cm, sibling distance=75mm]{node (s6) {$M_8$}
    child[level distance=1.3cm, sibling distance=20mm]{node {$x_8$}}
    child[sibling distance=30mm, level distance=1.3cm]{node (l2) {$x_9$ }}
    }
    };
%% Place gates and other symbols
%% In the CVS version of PGF labels are placed differently than in PGF 2.0
%% To render them correctly replace '-20' with 'right' and add the 'absolute'
%% option to the tikzpicture environment. The absolute option makes the 
%% node labels ignore the rotation of the parent node.
    \node [or] at (g1.south) [] {};
    \node [or] at (g2.south) [] {};
    \node [or] at (g3.south) [] {};
        %\draw[>=latex,->] (g3.north) to (g3.south);
    %\node [or] at (g3.south) [] {};
    \node [or] at (t1.south) [] {};
        % \draw[>=latex,->] (t1.north) to (t1.south);
    \node [and] at (t3.south) [] {};
    %\node [or] at (t2.south) [] {};
    \node [and] at (t2.south) (t2) [] {};
    %   \draw[>=latex,->] (t2.north) to (t2.south);
    % \node [and] at (s5.south) [] {};
        % \draw[>=latex,->] (s5.north) to (s5.south);
       \node [and] at (t4.south) (t4) [] {};
        \draw[>=latex,->] (t4.north) to (t4.south);  
        \node [or] at (l1.south) [] {};
    \node [or] at (s6.south) [] {};
        % \draw[>=latex,->] (s6.north) to (s6.south);
    %\node [or] at (s4.south) [] {};
    %\node [or] at (s7.south) [] {};
\end{tikzpicture}
\end{adjustbox}
\caption{{Risk model derived from the attack tree.}}
\label{fig:model}
\vspace{3mm}

==> TikzGraphs/DesignPrinciples1.tex <==
\centering
\resizebox{\linewidth}{!}
{ 
\begin{tikzpicture}
\begin{axis}[
    xlabel={Time (s)},
    ylabel={Probability of LoI},
      width=13cm, height=5.4cm,
    xmin=0, xmax=180,
    ymin=0, ymax=1.01,
%    xtick={30,40,50,60,70,80,90,100,110,120,130,140,150,160,170,180},
    xtick={0,20,40,60,80,100,120,140,160,180},
    ytick={0,0.2,0.4,0.6,0.8,1.0,1.08},
    legend pos= south east,
    ymajorgrids=true,
    grid style=dashed,
]
 
\addplot[
    color=green,
    mark=halfcircle,
    ]
    coordinates {
    (0,0) %(10,0.591) 
    (20,0.40) %(30,0.9204) 
    (40, 0.55) %(50, 0.949) 
    (60, 0.70) %(70,0.949) 
    (80, 0.75) %(90,0.95001) 
    (100, 0.8324) %(110, 0.95001) 
    (120, 0.8324) %(130, 0.95001) 
    (140, 0.8324) %(150, 1) 
    (160, 0.85) (180,0.85)
};
%coordinates {
    %(10,0.59) (20,0.82) (30,0.92) (40, 0.95) (50, 0.95) (60, 0.95) (70,0.95) (80,0.95) (90,1) (100, 1) (110, 1) (120, 1) (130, 1) (140, 1) (150, 1) (160, 1)

\addplot[
    color=magenta,
    mark=square,
    ]
    coordinates {
    (0,0) %(10,0.081) 
    (20,0.1804) %(30,0.235) 
    (40, 0.250) %(50, 0.387) 
    (60, 0.34) %(70,0.523) 
    (80, 0.52) %(90,0.654) 
    (100, 0.634) %(110, 0.743) 
    (120, 0.634) %(130,0.8) 
    (140, 0.634) %(150, 0.864) 
    (160, 0.646) (180,0.646)
};
    
   {\fontfamily{phv}\selectfont
\legend{Prob. before applying \textit{design principles}, Prob. after applying \textit{design principles}}
}
    
\end{axis}
\end{tikzpicture}
\label{fig:2design}
}
\label{fig:2design}
%\captionsetup{justification=centering}
%\caption{\scriptsize{Prob. of privacy leakage reduced by 68\%}}  
%\label{Diversity}     

==> TikzGraphs/DesignPrinciples2.tex <==
\centering
\resizebox{\linewidth}{!}
{ 
\begin{tikzpicture}
\begin{axis}[
    xlabel={Time (s)},
    ylabel={Probability of LoC},
      width=13cm, height=5.4cm,
    xmin=0, xmax=180,
    ymin=0, ymax=1.01,
%    xtick={30,40,50,60,70,80,90,100,110,120,130,140,150,160,170,180},
    xtick={0,20,40,60,80,100,120,140,160,180},
    ytick={0,0.2,0.4,0.6,0.8,1.0,1.08},
    legend pos= south east,
    ymajorgrids=true,
    grid style=dashed,
]
 
\addplot[
    color=green,
    mark=square,
    ]
    coordinates {
    (0,0) %(10,0.591) 
    (20,0.8524) %(30,0.9204) 
    (40, 0.9296) %(50, 0.949) 
    (60, 0.939) %(70,0.949) 
    (80,0.94001) %(90,0.95001) 
    (100, 0.94001) %(110, 0.95001) 
    (120, 0.94001) %(130, 0.95001) 
    (140, 0.94001) %(150, 1) 
    (160, 1) (180,1)
};
%coordinates {
    %(10,0.59) (20,0.82) (30,0.92) (40, 0.95) (50, 0.95) (60, 0.95) (70,0.95) (80,0.95) (90,1) (100, 1) (110, 1) (120, 1) (130, 1) (140, 1) (150, 1) (160, 1)

\addplot[
    color=magenta,
    mark=square,
    ]
    coordinates {
   (0,0) %(10,0.081) 
    (20,0.064) %(30,0.235) 
    (40, 0.1105) %(50, 0.387) 
    (60, 0.149) %(70,0.523) 
    (80,0.263) %(90,0.654) 
    (100, 0.325) %(110, 0.743) 
    (120, 0.421) %(130,0.8) 
    (140, 0.491) %(150, 0.864) 
    (160, 0.541) (180,0.596)
};

% coordinates {
%     (0,0) (10,0.045) (20,0.056) (30,0.10) (40, 0.12) (50, 0.14) (60, 0.15) (70,0.17) (80,0.25) (90,0.27) (100, 0.34) (110, 0.35) (120, 0.4) (130, 0.42) (140, 0.45) (150, 0.52) (160, 0.55) (180,0.56)
% };

    
    \legend{Prob. before applying \textit{design principles}, Prob. after applying \textit{design principles}}
\end{axis}
\end{tikzpicture}
}
\label{fig:3design}
%\captionsetup{justification=centering}
%\caption{\scriptsize{Prob. of privacy leakage reduced by 68\%}}  
%\label{Diversity}     

==> TikzGraphs/LoAdesignprinciple.tex <==
\centering
\resizebox{\linewidth}{!}
{ 
\begin{tikzpicture}
\begin{axis}[
    xlabel={Time (s)},
    ylabel={Probability of LoA},
      width=13cm, height=5.4cm,
    xmin=0, xmax=180,
    ymin=0, ymax=1.01,
%    xtick={30,40,50,60,70,80,90,100,110,120,130,140,150,160,170,180},
    xtick={0,20,40,60,80,100,120,140,160,180},
    ytick={0,0.2,0.4,0.6,0.8,1.0,1.08},
    legend pos= south east,
    ymajorgrids=true,
    grid style=dashed,
]
 
\addplot[
    color=green,
    mark=square,
    ]
    coordinates {
    (0,0) %(10,0.591) 
    (20,0.8524) %(30,0.9204) 
    (40, 0.9096) %(50, 0.949) 
    (60, 0.929) %(70,0.949) 
    (80,0.94001) %(90,0.95001) 
    (100, 0.96001) %(110, 0.95001) 
    (120, 0.96001) %(130, 0.95001) 
    (140, 0.96001) %(150, 1) 
    (160, 1) (180,1)
};
%coordinates {
    %(10,0.59) (20,0.82) (30,0.92) (40, 0.95) (50, 0.95) (60, 0.95) (70,0.95) (80,0.95) (90,1) (100, 1) (110, 1) (120, 1) (130, 1) (140, 1) (150, 1) (160, 1)

\addplot[
    color=magenta,
    mark=square,
    ]
    coordinates {
   (0,0) %(10,0.081) 
    (20,0.064) %(30,0.235) 
    (40, 0.1105) %(50, 0.387) 
    (60, 0.149) %(70,0.523) 
    (80,0.263) %(90,0.654) 
    (100, 0.325) %(110, 0.743) 
    (120, 0.421) %(130,0.8) 
    (140, 0.491) %(150, 0.864) 
    (160, 0.541) (180,0.596)
};

% coordinates {
%     (0,0) (10,0.045) (20,0.056) (30,0.10) (40, 0.12) (50, 0.14) (60, 0.15) (70,0.17) (80,0.25) (90,0.27) (100, 0.34) (110, 0.35) (120, 0.4) (130, 0.42) (140, 0.45) (150, 0.52) (160, 0.55) (180,0.56)
% };

    
    \legend{Prob. before applying \textit{design principles}, Prob. after applying \textit{design principles}}
\end{axis}
\end{tikzpicture}
}
\label{fig:LoAdesign}
%\captionsetup{justification=centering}
%\caption{\scriptsize{Prob. of privacy leakage reduced by 68\%}}  
%\label{Diversity}     

==> TikzGraphs/RiskScore.tex <==
\centering
\resizebox{\linewidth}{!}
{ 
\begin{tikzpicture}
\begin{axis}[
    xlabel={Number of Claims},
    ylabel={Risk Score of Claims},
      width=13cm, height=5.4cm,
    xmin=0, xmax=1000,
    ymin=0, ymax=10,
%    xtick={30,40,50,60,70,80,90,100,110,120,130,140,150,160,170,180},
    xtick={0,200,400,600,800,1000},
    ytick={0,2,4,6,8,10},
    legend pos= south east,
    ymajorgrids=true,
    grid style=dashed,
]
 
\addplot[
    color=green,
    mark=square,
    ]
    coordinates {
    (0,0) %(10,0.591) 
    (200,4) %(30,0.9204) 
    (400, 6) %(50, 0.949) 
    (600, 8) %(70,0.949) 
    (800, 8)
    (1000,9)
     
    
};
%coordinates {
    %(10,0.59) (20,0.82) (30,0.92) (40, 0.95) (50, 0.95) (60, 0.95) (70,0.95) (80,0.95) (90,1) (100, 1) (110, 1) (120, 1) (130, 1) (140, 1) (150, 1) (160, 1)

\addplot[
    color=magenta,
    mark=square,
    ]
    coordinates {
(0,0) %(10,0.591) 
    (200,3.2) %(30,0.9204) 
    (400, 4.9) %(50, 0.949) 
    (600, 5.2) %(70,0.949) 
    (800, 5.9)
    (1000,6.5)
};
    
    \legend{Prob. before applying \textit{design principles}, Prob. after applying \textit{design principles}}
\end{axis}
\end{tikzpicture}
\label{fig:2design}
}
\label{fig:2design}
%\captionsetup{justification=centering}
%\caption{\scriptsize{Prob. of privacy leakage reduced by 68\%}}  
%\label{Diversity}     
